Emergent Temporal Correspondences from Video Diffusion Transformers

Recent advancements in video diffusion models based on Diffusion Transformers (DiTs) have achieved remarkable success in generating temporally coherent videos. Yet, a fundamental question persists: how do these models internally establish and represent temporal correspondences across frames? We introduce DiffTrack, the first quantitative analysis framework designed to answer this question. DiffTrack constructs a dataset of prompt-generated video with pseudo ground-truth tracking annotations and proposes novel evaluation metrics to systematically analyze how each component within the full 3D attention mechanism of DiTs (e.g., representations, layers, and timesteps) contributes to establishing temporal correspondences. Our analysis reveals that query-key similarities in specific, but not all, layers play a critical role in temporal matching, and that this matching becomes increasingly prominent during the denoising process. We demonstrate practical applications of DiffTrack in zero-shot point tracking, where it achieves state-of-the-art performance compared to existing vision foundation and self-supervised video models. Further, we extend our findings to motion-enhanced video generation with a novel guidance method that improves temporal consistency of generated videos without additional training. We believe our work offers crucial insights into the inner workings of video DiTs and establishes a foundation for further research and applications leveraging their temporal understanding.

==> preamble.tex <==
\NeedsTeXFormat{LaTeX2e}
\RequirePackage{amsmath}
\RequirePackage{ifthen}
\RequirePackage{xspace}

% abbreviations
\providecommand*{\onedot}{\futurelet\@let@token\@onedot}
\providecommand*{\myonedot}{\ifx\@let@token.\else.\null\fi\xspace}

% abbreviations
\providecommand*{\eg}{\emph{e.g.}\xspace}
\providecommand*{\Eg}{\emph{E.g.}\xspace}
\providecommand*{\cf}{\emph{cf.}\xspace}
\providecommand*{\vs}{\emph{vs.}\xspace}
\providecommand*{\ie}{\emph{i.e.}\xspace}
\providecommand*{\Ie}{\emph{I.e.}\xspace}
\providecommand*{\iid}{\emph{i.i.d.}\xspace}
\providecommand*{\etc}{\emph{etc.}\xspace}
\providecommand*{\wrt}{\emph{w.r.t.}\xspace}
\providecommand*{\etal}{\emph{et~al.}\xspace}
\providecommand*{\lt}{\ensuremath{<}}
\providecommand*{\gt}{\ensuremath{>}}

\newcommand{\figureaftercaption}{\vspace{-3pt}}
\newcommand{\tablebeforecaption}{}
\newcommand{\tableaftercaption}{}

\AtEndPreamble{
    \usepackage[capitalize]{cleveref}
    \crefname{section}{Sec.}{Secs.}
    \Crefname{section}{Section}{Sections}
    \Crefname{table}{Table}{Tables}
    \crefname{table}{Tab.}{Tabs.}
}

\newif\ifdrafting
% \draftingtrue % To show comments
\draftingfalse % To hide comments

% --- inline annotations
\ifdrafting
    \newcommand{\red}[1]{{\color{red}#1}}
    \newcommand{\todo}[1]{{\color{red}#1}}
    \newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
    \newcommand{\jh}[1]{{\color{orange}[JH: #1]}}
\else
    % --- disable by uncommenting  
    \newcommand{\red}[1]{}
    \newcommand{\TODO}[1]{}
    \newcommand{\todo}[1]{#1}
    \newcommand{\jh}[1]{}
\fi
